PRoST: Distributed Execution of SPARQL Queries Using Mixed Partitioning Strategies

The rapidly growing size of RDF graphs in recent years necessitates distributed storage and parallel processing strategies. To obtain efficient query processing using computer clusters a wide variety of different approaches have been proposed. Related to the approach presented in the current paper are systems built on top of Hadoop HDFS, for example using Apache Accumulo or using Apache Spark. We present a new RDF store called PRoST (Partitioned RDF on Spark Tables) based on Apache Spark. PRoST introduces an innovative strategy that combines the Vertical Partitioning approach with the Property Table, two preexisting models for storing RDF datasets. We demonstrate that our proposal outperforms state-of-the-art systems w.r.t. the runtime for a wide range of query types and without any extensive precomputing phase.

==> chapters/1-introduction.tex <==
\section{Introduction}
Many organizations and projects, such as DBpedia \cite{auer2007dbpedia}, have adopted RDF to represent semantic data; the huge amount of information that can be collected has introduced the problem of storing and querying very large RDF graphs.\\
An RDF graph is a logical data model, but it can be stored physically using different techniques. Many approaches have been experimented to increase query efficiency: partitioning the data vertically \cite{abadi2007scalable} or with hash functions \cite{lee2013scaling}, introducing indexes \cite{punnoose2012rya} and precomputing some of the joins intermediate results \cite{schatzle2016s2rdf}.
Most of the current solutions use DBMS-based systems to store RDF graphs, mapping \textit{SPARQL} to SQL for querying. Some of them are implemented for single node machines, e.g. RDF-3X \cite{neumann2008rdf}, Sesame \cite{broekstra2002sesame} and Jena \cite{wilkinson2006jena}. Since computer clusters enable the possibility to scale up the storage for very large data and potentially increase parallelism, other solutions are implemented in distributed environments, in particular with Hadoop tools, e.g. S2RDF \cite{schatzle2016s2rdf} and SPARQLGX \cite{graux2016sparqlgx} on top of Apache Spark, Rya \cite{punnoose2012rya} on Apache Accumulo and Sempala \cite{schatzle2014sempala} on Impala.\\
We focus mainly on Apache Spark\footnote{https://spark.apache.org}, an important piece of the Hadoop ecosystem. It offers general purpose data processing functions that exploit efficiently the main memory, differently from MapReduce that relies mainly on disk. This characteristic makes Spark very fast in practise and able to compute complex queries on large RDF graphs.
In particular, it is possible to obtain high querying performances using Spark SQL, a module of Spark that adds well-established DBMS techniques to the distributed computation features.\\
The main goal of this work is to describe the approach of \textbf{PRoST} (Partitioned RDF on Spark Tables), that aims to improve the efficiency of RDF queries.
Instead of building a fully custom system, such as AdPart \cite{abdelaziz2017combining}, PRoST is based on reliable Hadoop technologies for storing and processing the data.
Our main contribution is to define an new storage organization for loading RDF graphs into Hadoop. 
%This model should not be intricate, but effective in solving some of the other systems' shortcomings. 
We want to prove that the combination of Vertical Partitioning with the Property Table, two preexisting data models, is reasonable to implement and, at the same time, it yields good querying performances.
As a consequence of the new model, we need to design a strategy to translate \textit{SPARQL} queries into execution plans .
Finally, it is necessary to evaluate PRoST in a real cluster using a large dataset and a range of diverse queries.\\
%%%%%%%%% STRUCTURE:
The paper is structured as follows:
in Section~\ref{sec:relatedwork} we present an overview of similar systems for RDF on Hadoop, in Section~\ref{sec:approach} we
outline our approach for modeling the data and our strategy to translate \textit{SPARQL} queries;
in Section~\ref{sec:optimization}, we show the most relevant techniques that we used to improve the performances of PRoST;
Section~\ref{sec:experiments} summarizes the evaluation results for our system, we assess different strategies that we used and we compare the performances with other systems;
finally, in Section~\ref{sec:conclusionfuturework}, we summarize our work and try to give ideas for future implementations of PRoST.



==> chapters/2-relatedwork.tex <==
\section{Related work}
\label{sec:relatedwork}
%\todo{Are these all comprable sytems to Prost? There are not so many! Maybe group the approaches (clusters, so create paragraph headers), or create a table with the most important characteristics and differences.}
\todo{if possible with the space, add other systems}\\
%%\subsection{S2RDF}
S2RDF \cite{schatzle2016s2rdf} is a "SPARQL processor" based on Spark SQL. It introduces a data partitioning approach that extends Vertical Partitioning \cite{abadi2007scalable} with additional tables, containing precomputed semi-joins.
As a consequence, many intermediate results of queries are already computed and they can be used to shorten the computing time. 
However, S2RDF trades off the performances with disk space and loading time. For datasets with a large number of properties (e.g. DBpedia \cite{auer2007dbpedia}), the time required makes the loading unfeasible.

%%\subsection{SPARQLGX}
SPARQLGX \cite{graux2016sparqlgx} is another system for distributed \textit{SPARQL} queries that uses Vertical Partitioning. SPARQLGX compiles the queries directly into Spark operations. The system relies entirely on its own statistics to optimize the computation, in particular for the order of the joins. Differently from S2RDF and PRoST, SPARQLGX does not use Spark SQL.
In \cite{graux2016sparqlgx}, the authors of SPARQLGX compare their system with S2RDF but oddly their evaluation seems not consistent with our experiments.

%%\subsection{Rya}
Rya \cite{punnoose2012rya} is a popular RDF management system, developed by an active open-source community and  currently an incubating project at Apache.
It is built on top of Apache Accumulo\footnote{https://accumulo.apache.org/}, a distributed key-value datastore for Hadoop. Since Accumulo keeps all its information sorted and indexed by key, Rya stores whole RDF triples as keys. For this reason, single triples or short ranges can be accessed very fast.
However, considering that the triple table model of Rya contains three columns, it requires to replicate the data multiple times in order to exploit the indexes over all the possible elements.
Rya uses some query optimization, e.g. joins reordering, but it lacks of the powerful in-memory data processing that make, in practise, other systems faster. 

==> chapters/3-approach.tex <==
\section{Approach}
\label{sec:approach}
The main idea behind PRoST is to store the data twice, partitioned in two different ways. Each one of the two data models can be more  beneficial than the other to the performances of certain types of queries, mainly because of the different location of the data in the cluster. Our system tries to exploit this characteristic. 
We did not limit ourselves to choosing the single best data model for each query, but we split a query in several parts, such that each sub-query can be executed with the most appropriate approach. At the end, all the parts can be joined together to produce the final results. In this way, not only we get good performances on a wider range of queries, but also we improve the outcome for those types that we believed were the prerogative of only one model at the time.

\subsection{Data model}\label{datamodels}
The two data models we use to store an RDF graph are \textit{Vertical Partitioning} and \textit{Property Table}.\\
\textit{Vertical Partitioning} (VP) is an approach proposed by Abadi et al.\cite{abadi2007scalable}, it has a strong popularity among RDF storage systems and it is the main choice of S2RDF\cite{schatzle2016s2rdf} and SPARQLGX\cite{graux2016sparqlgx}.
The main concept is to create a table for each distinct predicate of the input graph, containing all the tuples (subject, object) that are connected by that predicate. 
%VP tables can reduce the data size and it can be very beneficial to certain types of queries but they require also many joins between different tables.
The vertical partitioning approach is at the same time powerful and simple, but it has the drawback that it needs a number of joins equal to the number of triples in the query\footnote{To be precise, the number of triples minus one.}. Even with this disadvantage, because the VP tables are narrow and often small, VP is a valid and practical choice.\\
The \textit{Property Table} (PT) is a data scheme that was introduced in the implementation of Jena2 \cite{wilkinson2006jena}, an influential toolkit for RDF graphs, and Sempala \cite{schatzle2014sempala}, another \textit{SPARQL} processor built on top of the Impala framework. 
The PT consists of an unique table where each row contains a distinct subject and all the object values for that subject, stored in columns identified by the property to which they belong.\\
The most important advantage of this approach, if compared with VP, is that several joins can be avoided when some of the triple patterns in a query share the same subject. In this case, part of the query can be executed by a simpler select operator. Therefore, this approach is beneficial for queries where all the triple patterns have the same subject variable, usually called \textit{star} queries.
However, as observed by Abadi et al \cite{abadi2007scalable}, the PT has some issues, in particular the number of NULLs and the multi-valued attributes. Since not every possible pair subject-predicate has a corresponding object value, the PT potentially contains a very large number of NULLs. We solve this problem by storing the table in \textit{Parquet}\footnote{http://parquet.apache.org}, a format that uses run-length encoding. 
The other problem of the PT is the presence of multi-valued properties, when more than one different object value exists for at least one subject. In this case, the values are stored using lists that need to be flattened when executing operations on these attributes. This particular situation produces an overhead in respect to the VP model, significant if we use the PT for a single attribute, but negligible if compared to the benefit of avoiding more than one join to compute the same query.\\
We have several advantages (e.g. efficient compression) in using the columnar format \textit{Parquet} to store the PT, but we introduce also the undesirable possibility that the data belonging to a single subject could be split into different nodes. In order to keep benefiting from the structure of the property table, we partition horizontally on the subject column. In this way, we are sure that every row is stored entirely in the same node.

\subsection{Query strategies}\label{querystrategies}
Having two data models at the same time requires an abstraction to represent the queries. For this reason, we define an intermediate format that we call \textit{Join Tree}. Each node of this tree represents a sub-query extracted from a VP table or from the PT, and an edge between two nodes is a join between them. Using Spark, PRoST can execute a query by calculating the intermediate results from the nodes and then joining them together.\\
We need to explain how we translate \textit{SPARQL} queries into the \textit{Join Tree} format.
For the sake of clarity, we consider queries with a unique \textit{basic graph pattern} without filter, that is a conjunction of triple patterns.
The triple patterns with the same subject are grouped together and translated into a single node with a special label, denoting that we should use the property table in this case. All the other groups with a single triple pattern are translated to nodes that will use the vertical partitioning tables. An example is shown in Figure \ref{fig:joinTree_PT}.\\
There could be a join edge between every pair of nodes that shares a variable, it means that more than one  \textit{Join Tree} translation is possible for a single query. Since the tree structure influences the final performances, choosing carefully the \textit{Join Tree} is important for the quality of the system. For this reason, we choose a tree guided by simple statistics, as explained in the following section.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/implementation/triplesToTree.eps}
    \caption{Example of a conjunction of triple patterns translated to a Join Tree. The root node uses the Property Table, the others Vertical Partitioning.}
    \label{fig:joinTree_PT}
\end{figure}

\subsection{Statistics based optimization}
\label{sec:optimization}
In the context of our work, joins are the most expensive operators because they need large portion of the data to be shuffled across the network.
The order of the joins is important to limit this issue, and therefore to speed up the calculation. An effective way is sorting the joins using statistics of the input graph.
The \textit{Join Tree} of a query decides indirectly the order in which the operations are computed. For example, the leaves are computed first, and the root node is the final one.\\
The statistics we use, simple but effective in practise, are: the total number of triples and the number of distinct subjects for each predicate.
As a general rule of thumb, we want to compute the joins involving few data or with an high selectivity first (high priority), and finally the ones with many tuples (low priority).
The priority value of a node of the Join Tree is decided by these criteria:
\begin{itemize}
  \item Triple patterns containing literals are scored with the highest priority. The presence of a literal is a strong constraint that limit the number of resulting tuples. Therefore, it is a good approach to push down these kind of nodes.
  \item A triple of which the underlying data contains many tuples will be scored proportionally. For instance, a triple with the highest number of tuples will have also the lowest priority and it will be the root of the tree. This number is also adjusted according the number of distinct subjects for that predicate.
  \item The priority of a node containing data belonging to the Property Table is scored taking in account all its triple patterns. However, the presence of a triple pattern with a literal is weighted heavily.
\end{itemize}
In addition to our effort, Spark SQL’s Catalyst Optimizer \cite{armbrust2015spark} uses its internal heuristics to improve query performances further. The trees we define are not substantially changed, but Spark intervenes in producing optimized physical plans, since it knows the concrete location of the data on the cluster.
\todo{add an example of this optimizations}

==> chapters/4-experiments.tex <==
\section{Evaluation results}
\label{sec:experiments}

\subsection{Benchmark Environment}
We perform our tests on a small cluster of 10 machines connected via Gigabit Ethernet connection. Each machine is equipped with 32GB of memory, 4TB of disk space and with a 6 Core Intel Xeon E5-2420 processor. 
The cluster runs Cloudera CDH 5.11.0 on Ubuntu 14.04 and Spark 2.1.0. Since one machine is the master, Spark uses only 9 workers. The executor's memory is 21GB.\\
We use the WatDiv\cite{alucc2014diversified} dataset provided by the Waterloo SPARQL Diversity Test Suite 7. It is developed in order to measure how a RDF data management system performs across a wide variety of SPARQL queries with varying characteristics.\\
From WatDiv we generate a dataset containing around 100 Million triples and we evaluate PRoST with the given WatDiv Basic query set. It contains queries of varying shape and selectivity. The queries are grouped into the following subsets:
\begin{itemize}
    \item \textbf{C}: Complex shaped queries.
    \item \textbf{F (F1, F2, F3, F4, F5)}: Snowflake shaped queries.
    \item \textbf{L (L1, L2, L3, L4, L5)}: Linear shaped queries.
    \item \textbf{S (S1, S2, S3, S4, S5, S6, S7)}: Star shaped queries. 
\end{itemize}

\subsection{Loading}
As we can see from Table \ref{tab:loadingOtherSystems}, the size of the RDF graph decreases when stored in HDFS. This is a direct consequence of the compression used by the \textit{Parquet} format.
\begin{table}[tbh]
\begin{center}
    \begin{tabular}{|l|r|r|r|}
        \hline
        \textbf{System}  & \textbf{Size} & \textbf{Time}\\ \hline \hline
        PRoST & 2.1GB & 25m 32s\\
        SPARQLGX & 941MB & 20m 01s\\
        S2RDF & 6.2GB & 3h 11m 44s\\
        Rya & 3.1GB & 41m 32s\\
        \hline
    \end{tabular}
    \end{center}
    \caption[Table caption]{ Size and loading times using WatDiv100M}
    \label{tab:loadingOtherSystems}
\end{table}
The database size of S2RDF is the largest in this analysis, since its model not only needs the creation of VP tables, but also many additional ones containing the results of its precomputations. SPARQLGX occupies minimal space because it uses only Vertical Partitioning, where instead PRoST requires double SPARQLGX's size for having in addition the Property Table.
The loading time of PRoST is similar to SPARQLGX and around an order of magnitude shorter than S2RDF. Similarly to what we said before for the database size, S2RDF's model requires longer times because of its complicate precomputations.

\subsection{Vertical Partitioning vs Mixed Strategy}
One of our central points is the introduction of the Property Table alongside Vertical Partitioning. As a consequence, we evaluated the impact of this addition on query performances.\\
In Figure \ref{fig:VPvsPT} we show the times to evaluate the query set from WatDiv100M with Vertical Partitioning only and with the support of the Property Table.
\begin{figure}[tbh]
    \centering
    \includegraphics[width=\linewidth]{figures/experiments/mixed_vs_VP.eps}
    \caption{Querying time for WatDiv100M with only Vertical Partitioning and with the Mixed Strategy}
    \label{fig:VPvsPT}
\end{figure}
\noindent
The chart shows clearly how the introduction of the Property Table has a strong positive impact on performances. For almost every type of query this version outperforms abundantly the simple Vertical Partitioning approach.
The new strategy is effective for Star queries(S), where most of the triples share the same subject, as well as Complex (C) and Snowflake (F) queries, that have more than one different subject.
For some of the Linear queries (L), the results are very similar between the two versions. This result comes from the fact that Linear queries contain mostly triples with distinct subject variables, translated anyway using mostly Vertical Partitioning.\\
 
\subsection{PRoST vs other systems}
To better evaluate our system we compared it in the same environment with other similar solutions: S2RDF, Rya and SPARQLGX.\\
In Figure \ref{fig:resFFA} we show the querying times on the WatDiv100M dataset with the other systems and our implementation.
It is important to notice that we used a logarithmic scale, since the large differences would prevent us from well visualizing these results.
Compared to S2RDF, PRoST is faster for the queries L2, L5 and S3 but slower, even with a small difference, for all the other queries. In particular, for the complex queries (C) and some of the snowflake ones (F3, F4) the S2RDF's approach makes it faster by a consistent margin. These differences can be explained with the extensive precomputations of S2RDF, that heavily decrease the processing time for joins between VP tables. Anyhow, it is important to keep in mind that S2RDF can reach these results because of a very large loading time, that, for some datasets, makes it unusable in practise. On the contrary, PRoST relies on a faster loading phase and its performances do not depend on the particular input graph.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/experiments/all_results.eps}
    \caption{Querying time for WatDiv100M with PRoST, S2RDF, Rya and SPARQLGX. The scale is logarithmic.}
    \label{fig:resFFA}
\end{figure}
For some queries, Rya is very fast and outperforms PRoST but in other cases it suffers from significant slowdowns, that are several orders of magnitude slower. The queries in which Rya performs very well have in common that their computation involves few intermediate results. As a matter of fact, Rya uses powerful indexing methods but it lacks of more sophisticated approaches to calculate joins.
For SPARQLGX, almost all the queries are computed in around twenty seconds, except the Complex ones (C) that have an higher number of resulting tuples. PRoST outperforms SPARQLGX in every case, mostly by around an order of magnitude. Since SPARQLGX uses simple vertical partitioning, this difference confirms further the improvements produced by the introduction of the new data model and also increases the validity of the implementation choiches of PRoST.\\

==> chapters/5-conclusion_futurework.tex <==
\section{Conclusion and future work}
\label{sec:conclusionfuturework}

%%%\section{Summary}
We presented PRoST, a distributed system for RDF storage and \textit{SPARQL} querying built on top of Apache Spark. We introduced an innovative data model for partitioning RDF graphs that combines together two preexisting approaches: Vertical Partitioning and the Property Table. 
The impact of this model on performances is significant and crucial for the overall quality of PRoST. To refine our results, we optimized further the system using join reordering strategies based on statistics.\\
We evaluated PRoST on a small Hadoop cluster with the WatDiv benchmark test suite and we compared our system with Rya, SPARQLGX and S2RDF other solutions for RDF storage and \textit{SPARQL} processing.

%%%\section{Future Work}
PRoST is not yet fully mature, the implementation has room for enhancements that could lead to significant improvements in performances. For representing the queries we use an intermediate representation and the flexibility of this abstraction opens to the opportunity of introducing new data models, that could be used all together in a seamless execution.
For example, a new possibility would be adding another Property Table where, instead of the subjects, the rows would be created around objects. This could be beneficial for triple patterns that share the same object. Another possible improvement would be to collect more precise statistics of the input dataset, in order to produce better trees.\\




==> figures/background/figSiamese.tex <==
\tikzset{weights/.pic={
         code={
            %\tikzset{scale=5/10}
            \newcommand{\x}{0}
            \newcommand{\xb}{\x+0.3}
            \newcommand{\xc}{\x+0.6}
            \newcommand{\hf}{1.25}  % height front
            \newcommand{\hb}{1}  % height back
            \newcommand{\w}{1.2}  % width
            \newcommand{\y}{3.25}
            \filldraw[fill=white] (\xc, \y) -- (\xc, \y+\hb) -- (\xc+\w, \y+\hf) -- (\xc+\w,\y-0.25) -- (\xc, \y);
            \filldraw[fill=white] (\xb, \y) -- (\xb, \y+\hb) -- (\xb+\w, \y+\hf) -- (\xb+\w, \y-0.25) -- (\xb, \y);
            \filldraw[fill=white] (\x, \y) -- (\x, \y+\hb) -- (\x+\w, \y+\hf) -- (\x+\w,\y-0.25) -- (\x, \y);
            \node at (\x + 0.66, \y + 0.5) {$\mathbf{W}, b$};
  }}
}

\begin{figure}[t]
    \begin{center}
    \begin{tikzpicture}
        %conv nets
        \draw (2,5) rectangle (7.5,7.5) node[label={[shift={(-33ex,-1ex)}, align = left]south east:convolutional \\network 2}] {};
        \draw (2,0) rectangle (7.5,2.5) node[label={[shift={(-33ex,-1ex)}, align = left]south east:convolutional \\ network 1}] {};
        
        % distance
        \draw[->,very thick] (7.5,1.25) -- (8.5,1.25);
        \draw[->,very thick] (7.5,6.25) -- (8.5,6.25);
        \draw (8.5,0) rectangle (10,7.5) node[pos=.5] {distance};

        % optimizer
        \draw[->,very thick] (12, 6) -- (12, 5.25);
        \draw (11, 6) rectangle (13, 7.5) node[pos=.5] {optimizer};

        % loss
        \draw[->,very thick] (10,3.75) -- (11,3.75);
        \draw (11, 2.75) rectangle (12.5, 5.25) node[pos=.5] {loss};
        
        % inputs
        \draw[->,very thick] (1,1.25) -- (2,1.25);
        \draw[->,very thick] (1,6.25) -- (2,6.25);
        \draw (-0.5,5) rectangle (1,7.5) node[pos=.5] {input 1};
        \draw (-0.5,0) rectangle (1,2.5) node[pos=.5] {input 2};

        % similarity label
        \draw[->,very thick] (11.75,-1) -- (11.75,2.75);
        \draw[-,very thick] (1,-1) -- (11.75,-1);
        \node at (0, -1) {similarity $y$};

        % weights
        \path (5,0) pic {weights}[opacity=0.8];
        \path (5,2.5) pic {weights}[opacity=0.3];
        \path (5,-2.5) pic {weights}[opacity=0.3];

        \draw[-, dotted, thick, opacity=0.5] (5.5,4.6) -- (5.5,5.4);
        \draw[-, dotted, thick, opacity=0.5] (5.5,2.8) -- (5.5, 2);
        

    \end{tikzpicture}
    \end{center}
    \caption[Structure of a siamese neural network]{\textbf{Structure of a siamese neural network.} The two convolutional networks share the weights $\mathbf{W}$ and biases $b$. The distance between the output vectors of the two networks is fed into the the contrastive loss function. The contrastive loss penalizes small or large distances, depending on the similarity label $y$.}
    \label{fig:Siamese}
\end{figure}
